Greedy Algorithm for Multiway Matching with Bounded Regret

In this paper we prove the efficacy of a simple greedy algorithm for a finite horizon online resource allocation/matching problem, when the corresponding static planning linear program (SPP) exhibits a non-degeneracy condition called the general position gap (GPG). The key intuition that we formalize is that the solution of the reward maximizing SPP is the same as a feasibility Linear Program restricted to the optimal basic activities, and under GPG this solution can be tracked with bounded regret by a greedy algorithm, i.e., without the commonly used technique of periodically resolving the SPP. The goal of the decision maker is to combine resources (from a finite set of resource types) into configurations (from a finite set of feasible configurations) where each configuration is specified by the number of resources consumed of each type and a reward. The resources are further subdivided into three types - offline (whose quantity is known and available at time 0), online-queueable (which arrive online and can be stored in a buffer), and online-nonqueueable (which arrive online and must be matched on arrival or lost). Under GRG we prove that, (i) our greedy algorithm gets bounded any-time regret of $\mathcal{O}(1/\epsilon_0)$ for matching reward ($\epsilon_0$ is a measure of the GPG) when no configuration contains both an online-queueable and an online-nonqueueable resource, and (ii) $\mathcal{O}(\log t)$ expected any-time regret otherwise (we also prove a matching lower bound). By considering the three types of resources, our matching framework encompasses several well-studied problems such as dynamic multi-sided matching, network revenue management, online stochastic packing, and multiclass queueing systems.

==> preamble/preamble.tex <==
\usepackage{epsfig}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{theorem}
\usepackage{comment}
\usepackage{multirow}
\usepackage{setspace}
\usepackage[compact]{titlesec}
%\onehalfspacing
%\doublespacing
%\linespread{1.1}
%\usepackage{euler}
\usepackage{comment}
\usepackage{version}
\usepackage{enumitem}
\usepackage{multirow,subfigure}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage[pagebackref=true, bookmarks]{hyperref}
\hypersetup{
%backref controls whether the bibliography has a list of backreferences
%to where the citaiton is used
backref,
pageanchor=true,
%plainpages=false,
%pdfpagelabels, % makes the status line page labels the same as latex ones
bookmarks,
bookmarksnumbered,
colorlinks=true,
%pdfborder=0 0 1,
%pdfpagemode=UseOutlines,
menubordercolor= [rgb]{0, 0, 1},
linkbordercolor= [rgb]{0, 1, 1},
citecolor = red,
linkcolor= blue}
\usepackage{url}
\usepackage[numbers, sort]{natbib}

\usepackage{my_definitions}

% This is the stuff for normal spacing
\makeatletter
 \setlength{\textwidth}{6.8in}
 \setlength{\oddsidemargin}{-0.1in}
 \setlength{\evensidemargin}{0in}
 \setlength{\topmargin}{0in}
 \setlength{\textheight}{8.7in}
 \setlength{\headheight}{0pt}
 \setlength{\headsep}{0pt}
 \setlength{\marginparwidth}{59pt}

 \setlength{\parindent}{0in}
 %\setlength{\parskip}{.1in}
 \setlength{\theorempreskipamount}{5pt plus 1pt minus 3pt}
 \setlength{\theorempostskipamount}{0pt}
 \setlength{\abovedisplayskip}{8pt plus 3pt minus 9pt}

% This is to prevent full page figures from moving to the end
\renewcommand{\topfraction}{1.0}


\renewcommand{\section}{\@startsection{section}{1}{0mm}%
                                   {2ex plus -1ex minus -.2ex}%
                                   {1.3ex plus .2ex}%
                                   {\normalfont\Large\bfseries}}%
 \renewcommand{\subsection}{\@startsection{subsection}{2}{0mm}%
                                     {1ex plus -1ex minus -.2ex}%
                                     {1ex plus .2ex }%
                                     {\normalfont\large\bfseries}}%
 \renewcommand{\subsubsection}{\@startsection{subsubsection}{3}{0mm}%
                                     {1ex plus -1ex minus -.2ex}%
                                     {1ex plus .2ex }%
                                     {\normalfont\normalsize\bfseries}}
 \renewcommand\paragraph{\@startsection{paragraph}{4}{0mm}%
                                    {1ex \@plus1ex \@minus.2ex}%
                                    {-1em}%
                                    {\normalfont\normalsize\bfseries}}
% \renewcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
%                                       {2.0ex \@plus1ex \@minus .2ex}%
%                                       {-1em}%
%                                      {\normalfont\normalsize\bfseries}}
\titlespacing{\section}{2pt}{*0}{*0}
\titlespacing{\subsection}{1pt}{*0}{*0}
\titlespacing{\subsubsection}{0pt}{*0}{*0}

\makeatother

\renewcommand{\theequation}{\arabic{equation}}

\abovedisplayskip=0pt
\belowdisplayskip=0pt
\abovedisplayshortskip=0pt
\belowdisplayshortskip=0pt

\allowdisplaybreaks

\graphicspath{{./figures/}}


